A Frequency-Domain Differential Corrector for Quasi-Periodic Trajectory Design and Analysis

This paper introduces the Frequency-Domain Differential Corrector (FDDC), a model-agnostic approach for constructing quasi-periodic orbits (QPOs) across a range of dynamical regimes. In contrast to existing methods that explicitly enforce an invariance condition in all frequency dimensions, the FDDC targets dominant spectral components identified through frequency-domain analysis. Leveraging frequency refinement strategies such as Laskar-Numerical Analysis of Fundamental Frequency (L-NAFF) and G\'omez-Mondelo-Sim\'o-Collocation (GMS-C), the method enables efficient and scalable generation of high-dimensional QPOs. The FDDC is demonstrated in both single- and multiple-shooting formulations. While the study focuses on the Earth-Moon system, the framework is broadly applicable to other celestial environments. Sample applications include Distant Retrograde Orbits (DROs), Elliptical Lunar Frozen Orbits (ELFOs), and Near Rectilinear Halo Orbits (NRHOs), illustrating constellation design and the recovery of analog solutions in higher-fidelity models. With its model-independent formulation and spectral targeting capabilities, FDDC offers a versatile tool for robust trajectory design and mission planning in complex dynamical systems.

==> text/old_text.tex <==
%% laskar
Then, at the $\idxA$-th step, \acrshort{laskar} aims to adjust $\freqA{\idxA}$ via satisfying,
\begin{align}
    \label{eq:laskar_condition}\freqA{\idxA} & = \argmax{\freqAArg} (|
    \signalf(\freqAArg)|)  \\
    \signalf(\freqAArg) & = \frac{1}{\sampleSize}\sum_{\idxT=0}^{\sampleSize-1} \signalt ( \tidxT)  \han(\idxT) \exp{-\imag  \freqAArg\tidxT} = \frac{1}{N}\sum_{\idxT}^{\sampleSize-1} \biggl( \signalt ( \tidxT)  \han(\idxT) \bigl( \cos (\freqAArg\tidxT )  - \imag \sin ( \freqAArg\tidxT) \bigr)\biggr) \\
    |\signalf(\freqAArg)| & = \frac{1}{2} \sqrt{\cosf(\freqAArg)^2 + \sinf(\freqAArg)^2} \\
    \cosf(\freqAArg)& = 2\text{Re} ( \signalf(\freqAArg)) = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  \signalt ( \tidxT)  \han(\idxT) \cos ( \freqAArg\tidxT)  \\
    \sinf(\freqAArg)& = -2\text{Im} ( \signalf(\freqAArg)) = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  \signalt ( \tidxT)  \han(\idxT) \sin ( \freqAArg\tidxT)   \\
    & \label{eq:signAmb} \freqP{\idxA} \leq \freqAArg \leq \freqPP{ \idxA}\; (|\signalf(\freqD{\idxF+1})| > |\signalf(\freqD{\idxF-1})| ) \quad \text{or} \quad \freqPM{\idxA} \leq \freqAArg \leq \freqP{ \idxA}\; (|\signalf(\freqD{\idxF+1})| \leq |\signalf(\freqD{\idxF-1})| ).
\end{align}
Note that $\freqP{\idxA}$ is the $\idxF$-th frequency associated with the $\idxA$-th peak within the \acrshort{dft} on $\signalt$. For algorithmic robustness, it is assumed that the true frequency lies between the $\idxA$-th and the nearby frequency, $\idxA\pm1$\us{check if this is true} where the sign is decided by the relative magnitude of the \acrshort{dft} amplitude. Then, the physical meaning of this condition from Eq. \eqref{eq:laskar_condition} is to enforce that the magnitude of a \acrshort{dft} on $\signalt$ with the frequency $\freqA{\idxA}$ to be maximized. The condition is also written as,
\begin{align}
    \label{eq:laskar_condition}\freqA{\idxA} & = \argmax{\freqAArg} (|
    \signalf(\freqAArg)|) \Rightarrow \\
    & \label{eq:laskar_f1} \frac{d |\signalf(\freqA{\idxA})|}{d \freqA{\idxA}}= \frac{1}{2\sqrt{\cosf(\freqA{\idxA})^2 + \sinf(\freqA{\idxA})^2}}\left(\cosf(\freqA{\idxA}) \frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}} + \sinf(\freqA{\idxA}) \frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}}  \right)   = 0.
\end{align}
Here, the derivatives for $\cosf(\freqA{\idxA})$ and $\sinf(\freqA{\idxA})$ are, 
\begin{align}
    \frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}} & = \frac{2}{N}\sum_{\idxT}^{\sampleSize-1}  \tidxT \signalt ( \tidxT)  \han(\idxT) (- \sin (\freqA{\idxA}\tidxT )) \\
    \frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}} & =  \frac{2}{N}\sum_{\idxT}^{\sampleSize-1} \tidxT \signalt ( \tidxT)  \han(\idxT) (\cos (\freqA{\idxA}\tidxT ) ).
\end{align}
Here, the first order condition implies the maximum as $\freqD{\idxA}$ is close to $\freqA{\idxA}$. For the amplitude and the phase, consider the \acrshort{dft} on the $\idxA$-th approximation for the signal, i.e., $ \signalaidxA(\tnd) = \ampA{\idxA} \cos (\freqA{\idxA} \tnd + \phaseA{\idxA}) = \ampA{\idxA} \cos \phaseA{\idxA}\cos (\freqA{\idxA}) - \ampA{\idxA} \sin \phaseA{\idxA}\sin (\freqA{\idxA})  $ evaluated at $\freqA{\idxA}$. Noting that,
\begin{align}
     \coscosf(\freqA{\idxA}) & = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  (\cos (\freqA{\idxA} \tidxT) )^2 \han(\idxT) \approx 1 \\
    \sincosf(\freqA{\idxA}) = \cossinf(\freqA{\idxA}) & = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  \cos (\freqA{\idxA} \tidxT)\sin (\freqA{\idxA}\tidxT ) \han(\idxT) \approx 0  \\
    \sinsinf(\freqA{\idxA})& = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  (\sin (\freqA{\idxA} \tidxT)) ^2\han(\idxT) \approx 1.
\end{align}
Although these numbers are close to either $1$ or $0$, they are not exactly constant due to discretization and the Hann window function. 
Also,
\begin{align}
    \dft{\signalaidxA}{\freqA{\idxA}} = \left[\frac{1}{2}\ampA{\idxA}\cos \phaseA{\idxA} \coscosf(\freqA{\idxA}) - \frac{1}{2}\ampA{\idxA}\sin \phaseA{\idxA} \cossinf(\freqA{\idxA})\right]  +\imag \left[-\frac{1}{2}  \ampA{\idxA}\cos \phaseA{\idxA}\sincosf(\freqA{\idxA}) + \frac{1}{2}  \ampA{\idxA}\sin \phaseA{\idxA}\sinsinf(\freqA{\idxA}) \right].
\end{align}
Here, it is desired that at the approximated frequency $\freqA{\idxA}$, the approximated signal $\signalaidxA$ and the true signal $\signalt$ demonstrate the same behavior, i.e.,
\begin{align}
    \dft{\signalaidxA}{\freqA{\idxA}} = \dft{\signalt}{\freqA{\idxA}}.
\end{align}
Thus, this condition results in two equations,
\begin{align}
    & \label{eq:laskar_f2} \ampA{\idxA}\cos \phaseA{\idxA}\coscosf(\freqA{\idxA})  - \ampA{\idxA}\sin \phaseA{\idxA} \cossinf(\freqA{\idxA})  = \cosf(\freqA{\idxA}) \\
    & \label{eq:laskar_f3} \ampA{\idxA}\cos \phaseA{\idxA}\sincosf(\freqA{\idxA})   - \ampA{\idxA}\sin \phaseA{\idxA} \sinsinf(\freqA{\idxA}) = \sinf(\freqA{\idxA}).
\end{align}
Starting from this initial guess, from Eqs. \eqref{eq:laskar_f1}-\eqref{eq:laskar_f3}, following constraint vector is enforced,
\begin{align}
    \label{eq:laskar_constraint} \constraintVL = \begin{bmatrix}
        \constraintC{L, \freqAArg} \\ \constraintC{L, \mathcal{C}} \\\constraintC{L, \mathcal{S}}  
    \end{bmatrix} = \begin{bmatrix}
        \frac{1}{2\sqrt{\cosf(\freqA{\idxA})^2 + \sinf(\freqA{\idxA})^2}}\left(\cosf(\freqA{\idxA}) \frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}} + \sinf(\freqA{\idxA}) \frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}}  \right) \\
        \ampA{\idxA}\cos \phaseA{\idxA}\coscosf(\freqA{\idxA})  - \ampA{\idxA}\sin \phaseA{\idxA} \cossinf(\freqA{\idxA})  - \cosf(\freqA{\idxA}) \\
    \ampA{\idxA}\cos \phaseA{\idxA}\sincosf(\freqA{\idxA})   - \ampA{\idxA}\sin \phaseA{\idxA} \sinsinf(\freqA{\idxA}) - \sinf(\freqA{\idxA}).
    \end{bmatrix} = \bar{0}.
\end{align}
The Jacobian of $ \constraintVL$ with respect to $\freeVL$ is rendered as,
\begin{align}
    \frac{\partial \constraintVL}{\partial \freeVL} = \begin{bmatrix}
    \frac{\partial \constraintC{L, \freqAArg}}{\partial \freqA{\idxA}} & \frac{\partial \constraintC{L, \freqAArg}}{\partial \ampA{\idxA}} & \frac{\partial \constraintC{L, \freqAArg}}{\partial \phaseA{\idxA}} \\
        \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \freqA{\idxA}} & \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \ampA{\idxA}} & \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \phaseA{\idxA}} \\
        \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \freqA{\idxA}} & \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \ampA{\idxA}} & \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \phaseA{\idxA}}
    \end{bmatrix},
\end{align}
with each component,
\begin{align}
    \frac{\partial \constraintC{L, \freqAArg}}{\partial \freqA{\idxA}} & = -\frac{1}{2\sqrt{\cosf(\freqA{\idxA})^2 + \sinf(\freqA{\idxA})^2}^3}\left(\cosf(\freqA{\idxA}) \frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}} + \sinf(\freqA{\idxA}) \frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}}  \right)^2 \nonumber \\
    & + \frac{1}{2\sqrt{\cosf(\freqA{\idxA})^2 + \sinf(\freqA{\idxA})^2}}\left(\left(\frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}}\right)^2 + \left(\frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}}\right)^2 + \cosf(\freqA{\idxA}) \frac{d^2 \cosf(\freqA{\idxA})}{d \freqA{\idxA}^2} + \sinf(\freqA{\idxA}) \frac{d^2 \sinf(\freqA{\idxA})}{d \freqA{\idxA}^2}  \right)\\
    \frac{\partial \constraintC{L, \freqAArg}}{\partial \ampA{\idxA}} & = 0 \\
    \frac{\partial \constraintC{L, \freqAArg}}{\partial \phaseA{\idxA}} & = 0\\
    \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \freqA{\idxA}} & =  \ampA{\idxA}\cos \phaseA{\idxA} \frac{d \coscosf(\freqA{\idxA})}{d \freqA{\idxA}} - \ampA{\idxA}\sin \phaseA{\idxA}\frac{d \cossinf(\freqA{\idxA})}{d \freqA{\idxA}}  - \frac{d \cosf(\freqA{\idxA})}{d \freqA{\idxA}} \\
    \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \ampA{\idxA}} &= \cos \phaseA{\idxA}\coscosf(\freqA{\idxA})  - \sin \phaseA{\idxA} \cossinf(\freqA{\idxA}) \\
    \frac{\partial \constraintC{L, \mathcal{C}}}{\partial \phaseA{\idxA}} &= -\ampA{\idxA}\sin \phaseA{\idxA}\coscosf(\freqA{\idxA})  - \ampA{\idxA}\cos \phaseA{\idxA} \cossinf(\freqA{\idxA})\\
    \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \freqA{\idxA}} & =  \ampA{\idxA}\cos \phaseA{\idxA}\frac{d \sincosf(\freqA{\idxA})}{d \freqA{\idxA}}  - \ampA{\idxA}\sin \phaseA{\idxA} \frac{d \sinsinf(\freqA{\idxA})}{d \freqA{\idxA}} - \frac{d \sinf(\freqA{\idxA})}{d \freqA{\idxA}} \\ 
    \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \ampA{\idxA}} &= \cos \phaseA{\idxA} \sincosf({\freqA{\idxA}}) - \sin \phaseA{\idxA}\sinsinf({\freqA{\idxA}})   \\
    \frac{\partial \constraintC{L, \mathcal{S}}}{\partial \phaseA{\idxA}} &= -\ampA{\idxA}\sin \phaseA{\idxA} \sincosf{(\freqA{\idxA})} - \ampA{\idxA}\cos \phaseA{\idxA} \sinsinf{(\freqA{\idxA})} .
\end{align}
Note the following additional quantities,
\begin{align}
   & \frac{d^2 \cosf(\freqA{\idxA})}{d \freqA{\idxA}^2} = \frac{2}{\sampleSize}\sum_{\idxT = 0}^{\sampleSize-1} \tidxT^2 \signalt(\tidxT) \han(\idxT) (- \cos (\freqA{\idxA}\tidxT )) \\
   & \frac{d^2 \sinf(\freqA{\idxA})}{d \freqA{\idxA}^2} = \frac{2}{\sampleSize}\sum_{\idxT = 0}^{\sampleSize-1} \tidxT^2 \signalt(\tidxT) \han(\idxT) (- \sin ( \freqA{\idxA}\tidxT)) \\
   & \frac{d \coscosf(\freqA{\idxA})}{d \freqA{\idxA}}  = -\frac{d \sinsinf(\freqA{\idxA})}{d \freqA{\idxA}} =  \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  (-2\tidxT \sin (\freqA{\idxA} \tidxT)   \cos (\tidxT \freqA{\idxA}) \han(\idxT))  \\
   & \frac{d\sincosf(\freqA{\idxA})}{d\freqA{\idxA}} = \frac{2}{\sampleSize}\sum_{\idxT}^{\sampleSize-1}  (-\tidxT (\sin (\freqA{\idxA}) )^2  \han(\idxT)  + \tidxT (\cos (\freqA{\idxA} \tidxT))^2  \han(\idxT)  ).
\end{align}
After $j$-th peak is converged, $(j+1)$-th peak is investigated. For robustness in the algorithm to detect subsequent peaks, it is possible to analyze the difference of the original signal to the $j$-th approximation, i.e., $\signalt^{new}_{\idxA} \coloneq \signalt - (\ampA{0} + \sum_{m=1}^{\idxA }\tilde{\signalt}^{m}$). In the new signal $\signalt^{new}_{\idxA}$, the $(\idxA+1)$-th peak from the original signal $\signalt$ is expected to occur as the first peak, facilitating the detection through the \acrshort{dft}. 

Partial derivatives for the remaining two constraints follow similar structure. The selection of $\mathcal{CS}$ at $\freqPO{\idxA}$

For refinement process, \acrshort{dft} on cosine and sine with the approximated frequency, $\freqA{\idxA}$, are leveraged,
\begin{align}
    \signalcosf(\fidxF) & = \frac{1}{\sampleSize}\sum_{\idxT=0}^{\sampleSize-1} \cos (\freqA{\idxA} \tidxT ) \han(\idxT) \exp{ - \imag  \fidxF \tidxT} \\
    \signalsinf(\fidxF) & = \frac{1}{\sampleSize}\sum_{\idxT=0}^{\sampleSize-1} \sin (\freqA{\idxA} \tidxT ) \han(\idxT) \exp{ - \imag  \fidxF \tidxT} \\
    \frac{d \signalcosf(\fidxF)}{d \freqA{\idxA}} & = \frac{1}{\sampleSize}\sum_{\idxT=0}^{\sampleSize-1} - \tidxT \sin (\freqA{\idxA} \tidxT ) \han(\idxT) \exp{ - \imag  \fidxF \tidxT} \\
    \frac{d \signalsinf(\fidxF)}{d \freqA{\idxA}}  & = \frac{1}{\sampleSize}\sum_{\idxT=0}^{\sampleSize-1} \tidxT \cos (\freqA{\idxA} \tidxT ) \han(\idxT) \exp{ - \imag  \fidxF \tidxT} 
\end{align}
where $c(\freqA{\idxA}), s(\freqA{\idxA})$ denote $\cos (\freqA{\idxA} \tnd), \sin (\freqA{\idxA} \tnd)$, respectively. Note that the same Hann window function and time step ($\tidxT$) are leveraged. Correspondingly, following notations are utilized,
\begin{align}
    \coscosf(\fidxF) & = 2 \text{Re}(\signalcosf(\fidxF)) \\
    \cossinf(\fidxF) & = 2 \text{Re}(\signalsinf(\fidxF)) \\
    \sincosf(\fidxF) & = -2 \text{Im}(\signalcosf(\fidxF)) \\
    \sinsinf(\fidxF) & = -2 \text{Im}(\signalsinf(\fidxF)) \\
    \frac{d\coscosf(\fidxF)}{d\freqA{\idxA}} & = 2 \text{Re}(\frac{d \signalcosf(\fidxF)}{d \freqA{\idxA}}) \\
    \frac{d\cossinf(\fidxF)}{d\freqA{\idxA}} & = 2 \text{Re}(\frac{d \signalsinf(\fidxF)}{d \freqA{\idxA}}) \\
    \frac{d\sincosf(\fidxF)}{d\freqA{\idxA}} & = -2 \text{Im}(\frac{d \signalcosf(\fidxF)}{d \freqA{\idxA}}) \\
    \frac{d\sinsinf(\fidxF)}{d\freqA{\idxA}} & = -2 \text{Im}(\frac{d \signalsinf(\fidxF)}{d \freqA{\idxA}}).
\end{align}


While \acrshort{laskar} directly optimizes for $\freqA{\idxA}$ through the maximum condition from Eq. \eqref{eq:laskar_f1}, \acrshort{gomez} achieves the refinement via introducing collocation constraints at frequencies $\freqP{\idxA}$ and $\freqP{\idxA\pm1}$. More specifically, following conditions are generally desired,
\begin{align}
    & \label{eq:k}\dft{\signalaidxA}{\freqP{\idxA}} = \dft{\signalt}{\freqP{\idxA}} \\
    & \label{eq:k+1}\dft{\signalaidxA}{\freqPO{\idxA}} = \dft{\signalt}{\freqPO{\idxA}}.
\end{align}
Here, the sign ambiguities are handled via Eq. \eqref{eq:signAmb}, i.e., the index that corresponds to larger \acrshort{dft} magnitude is selected. Still, the collocation results in four different equations for the general, three-dimensional free variable (Eq. \eqref{eq:freeV}), resulting in an over-constraint problem. To ensure an invertible Jacobian, only cosine or sine components are collocated for Eq. \eqref{eq:k+1}. Together, Eqs. \eqref{eq:k} and \eqref{eq:k+1} are expanded as,
\begin{align}
    \label{eq:gomez_constraint_idxA_both_side_1} & \ampA{\idxA}\cos\phaseA{\idxA} \coscosf(\freqP{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \cossinf(\freqP{\idxA}) = \cosf(\freqP{\idxA}) \\
    \label{eq:gomez_constraint_idxA_both_side_2} & \ampA{\idxA}\cos\phaseA{\idxA} \sincosf(\freqP{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \sinsinf(\freqP{\idxA}) = \sinf(\freqP{\idxA}) \\
    \label{eq:gomez_constraint_idxA_both_side_3} & \ampA{\idxA}\cos\phaseA{\idxA} \cscosf(\freqPO{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \cssinf(\freqPO{\idxA}) = \csf(\freqPO{\idxA}),
\end{align}
where $\mathcal{CS}$ denotes one of $\mathcal{C}$ or $\mathcal{S}$ is selected. Three collocation conditions are concatenated as,
\begin{align}
    \label{eq:gomez_constraint_idxA} \constraintVG = \begin{bmatrix}
        \constraintC{G, \mathcal{C}(\freqP{\idxA})} \\ 
        \constraintC{G, \mathcal{S}(\freqP{\idxA})} \\
        \constraintC{G, \mathcal{CS}(\freqPO{\idxA})}
    \end{bmatrix} = \begin{bmatrix}
        \ampA{\idxA}\cos\phaseA{\idxA} \coscosf(\freqP{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \cossinf(\freqP{\idxA}) - \cosf(\freqP{\idxA}) \\
        \ampA{\idxA}\cos\phaseA{\idxA} \sincosf(\freqP{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \sinsinf(\freqP{\idxA}) - \sinf(\freqP{\idxA}) \\
        \ampA{\idxA}\cos\phaseA{\idxA} \cscosf(\freqPO{\idxA}) - \ampA{\idxA}\sin\phaseA{\idxA} \cssinf(\freqPO{\idxA}) - \csf(\freqPO{\idxA})
    \end{bmatrix} = \bar{0}.
\end{align}

finement techniques, i.e., \acrshort{laskar} and \acrshort{gomez}, are similar in that both methods leverage auxiliary \acrshort{dft} to further refine the quasi-periodic approximations. The auxiliary \acrshort{dft} provide algebraic constraints, i.e., Eqs. \eqref{eq:laskar_constraint}-\eqref{eq:gomez_constraint_idxA} that are targeted via adjusting the free variable, Eq. \eqref{eq:freeV}. Note that the \textit{standard} \acrshort{dft} refers to the vector of \acrshort{dft} (Eq. \eqref{eq:dft}) on the signal ($\signalt$) at the frequency bins represented by Eq. \eqref{eq:bins}. Then, as the auxiliary \acrshort{dft}, \acrshort{laskar} leverages the \acrshort{dft} on the same signal, i.e., $\signalt$, but at the frequency generally does not coincide with the frequency bins, i.e., $\freqA{\idxA} \neq \fidxF$. In contrast, \acrshort{gomez} constructs \acrshort{dft} at the same frequency bins from the standard \acrshort{dft}, but now on distinct signals consisting of cosines and sines of $\freqA{\idxA}$. 






The results are illustrated in Figure \ref{fig:dro-compare-l-g-dft.png} with plot dots for each frequency bin, where the vertical axis illustrates the $\log_{10}$ of the amplitude associated with the \acrshort{dft}. Note that the peaks from the \acrshort{dft} are generally associated with multiples of $\freqAArg_C = 2\pi/1.6$, a value analytically determined from the nondimensional period of the orbit in Table \ref{table:dro_initial}. As the frequency bins from the \acrshort{dft}, i.e., $\freqD{\idxT}$, generally do not coincide with the multiples of $\freqAArg_C $, the two refinement algorithms (\acrshort{laskar} and \acrshort{gomez}) are employed to supply refined values for the peak frequencies. Then, Figure \ref{fig:dro-compare-l-g-refine.png} demonstrates the error of the peaks supplied by each algorithm as compared to the analytic value provided by $\freqAArg_C = 2\pi/1.6$ for each multiple. The markers do not appear for $1$. Both methods provide estimates with $\approx 0$ error. The detailed performance may differ in specific scenarios and are subject to muliplte factors, e.g., numerical formulation for the \acrshort{dft} signals and the sample size. For the current investigation, it is sufficient to note that for the dominant frequencies, \textbf{both methods supply reliable estimates for the true peak.} In subsequent sections and applications, both methods are utilized and are generally interchangeable. 




The current section focuses on dynamical regimes where instabilities do not exist. In such a case, the signal $\signalt$ is retrieved via propagating a single, initial six-dimensional state, $\x{0} \in \real{6}$. For an initial derivation of the algorithm, consider the autonomous Hamiltonian system as the dynamical model. In this region, at least locally, dense $\inter$-dimensional QPOs exist within the $\inter$ degree-of-freedom autonomous Hamiltonian systems.\footnote{While local instabilities potentially emanate from the resonant periodic orbits in the spatial case (Arnold diffusion \cite{arnol2013mathematical}), rate of the departure is demonstrated to be sufficiently slow \cite{morbidelli1995superexponential}.} Examples within the Earth-Moon \acrshort{cr3bp} include, but are not limited to, the \acrfull{dro} family and the \acrfull{elfos}. The \acrshort{fdc} in a single-shooting formulation adopts $\x{0}$ as the free variable and enforces following constraint, 
\begin{align}
    \f  = \begin{bmatrix} \freqA{\idxA} - \freqA{\idxA}^T \\ \phaseA{\idxA} - \phaseA{\idxA}^T \end{bmatrix} \quad \text{or} \quad \begin{bmatrix} \ampA{\idxA} - \ampA{\idxA}^T \\ \phaseA{\idxA} - \phaseA{\idxA}^T \end{bmatrix},
\end{align}
where the superscript $T$ denotes the target frequency information. Note that, for the quasi-periodic trajectories of interest, the frequency and amplitude, i.e., $\freqA{\idxA}, \ampA{\idxA}$, are coupled; attempting to target these two variables simultaneously results in an overconstrained problem in general. Thus, it is only possible to target either $\freqA{\idxA}$ or $\ampA{\idxA}$, where different formulation is suited better for different applications. To construct a differential corrector, the gradient of $\f$ with respect to $\x{0}$ is required. Such information requires the following derivatives,
\begin{align}
    \label{eq:fdt_partial_gomez_required} \frac{d \freqA{\idxA}}{d \x{0}}, \frac{d \ampA{\idxA}}{d \x{0}}, 
    \frac{d \phaseA{\idxA}}{d \x{0}} .
\end{align}
Note that the constraints from two frequency refinement strategies (Eqs. \eqref{eq:laskar_constraint} and \eqref{eq:gomez_constraint_idxA}) supply the algebraic relationships to supply these sensitivity vectors in Eq. \eqref{eq:fdt_partial_gomez_required}. These vectors are supplied for each refinement method in the subsequent sections. 


For these dynamical regime, any initial condition does not diverge from the local vicinity. The norm of the \acrfull{stm} also grows at a linear rate (linear since the generalize eigenvector exists that signifies the shift in phase), allowing a single-shooting formulation. Now, denote the initial condition as $\x{0}\in \real{6}$. It is possible that the dynamical model is time-dependent. In such a case, the initial epoch is constructed as $\epoch{0}$. The current analysis discusses this fixed-time formulation where $\epoch{0}$ does not vary. 






The Long-Period Frequency, $\nu_L$: While detecting and targeting $\nu_L$ follows similar steps as those used for $\nu_M$, additional complexities arise. First, for \acrshort{elfos} tracking 2D tori, the \acrshort{dft} cannot identify oscillations with non-zero amplitudes, as $\theta_L$ is poorly defined for these structures. For nearby structures close to the magenta surface in Fig. \ref{fig:3d_surface_constants_averaged}, long-period oscillations are associated with small amplitudes. Furthermore, $\nu_L$ is obviously associated with a small value, e.g., $\nu_L \approx 0.059$ [nd] for the 3D tori family plotted in Fig. \ref{fig:3d_surface_families}. Recall that the resolution of the \acrshort{dft} analysis is limited by $2\pi / t_{N-1}$. To ensure $\nu_L \gg 2\pi / t_{N-1}$ and facilitate detection, the total propagation time must span several decades, potentially leading to significant computational costs. Moreover, during extended propagation, the norm of the state transition matrix from Eq. \eqref{eq:stm} grows substantially, reducing the robustness of the frequency-targeting process. Note that the long-frequency $\nu_L$ governs the deviation from the \acrshort{elfos} (2D tori), where evolution in $\nu_L$ leads to invariant surface spanning wider area as plotted in Figs. \ref{fig:sample_propagation_2d_elfo_strobo_fft} and \ref{fig:3d_surface_families_3d_geometry}. In light of this observation, in practical applications, controlling the geometric deviation, $A_L$, may be more desirable than directly targeting $\nu_L$. Note that $A_L = A_L (\nu_S, \nu_M, \nu_L)$. Thus, the constraint vector is well-defined with $A_L$ in lieu of $\nu_L$ and serves as an alternative option to supply a square system with a six-dimensional vectors $\vec{\mathbb{X}}_0$ and $\vec{\mathbb{F}}(\vec{\mathbb{X}}_0)=\vec{0}$. With these additional complexities for targeting the long-period frequency $\nu_L$, $x$ position components within the \acrshort{brf} are leveraged to construct Eq. \eqref{eq:implicit}. 
